Unveiling Backbone Effects in CLIP: Exploring Representational Synergies and Variances

Contrastive Language-Image Pretraining (CLIP) stands out as a prominent method for image representation learning. Various neural architectures, spanning Transformer-based models like Vision Transformers (ViTs) to Convolutional Networks (ConvNets) like ResNets, are trained with CLIP and serve as universal backbones across diverse vision tasks. Despite utilizing the same data and training objectives, the effectiveness of representations learned by these architectures raises a critical question. Our investigation explores the differences in CLIP performance among these backbone architectures, revealing significant disparities in their classifications. Notably, normalizing these representations results in substantial performance variations. Our findings showcase a remarkable possible synergy between backbone predictions that could reach an improvement of over 20% through informed selection of the appropriate backbone. Moreover, we propose a simple, yet effective approach to combine predictions from multiple backbones, leading to a notable performance boost of up to 6.34\%. We will release the code for reproducing the results.

==> notations.tex <==
\newcommand{\ie}{\textit{i.e.}\xspace}
\newcommand{\eg}{\textit{e.g.}\xspace}

\newcommand{\bx}{\boldsymbol{x}}
\newcommand{\bxr}{\boldsymbol{\hat{x}}}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\bs}{\boldsymbol{s}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bkappa}{\boldsymbol{\kappa}}
\newcommand{\bt}{\boldsymbol{t}}
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\byr}{\boldsymbol{\hat{y}}}
\newcommand{\bX}{\mathcal{X}}
\newcommand{\bV}{\mathcal{V}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bT}{\mathcal{T}}
\newcommand{\bH}{\mathcal{H}}
\newcommand{\bD}{\mathbf{X}}
\newcommand{\bset}{\mathbf{D}}
\newcommand{\bsetU}{\mathbf{D}_{\text{uncertain}}}
\newcommand{\bDC}{\bD_{\text{confident}}}
\newcommand{\bDU}{\bD_{\text{uncertain}}}
\newcommand{\bDyR}{\bDy_{\text{refined}}}
\newcommand{\bDCbar}{{\bar{X}}_{\text{confident}}}
\newcommand{\bDy}{\bset}
\newcommand{\bDyU}{\bsetU}
\newcommand{\bA}{\mathcal{A}}
\newcommand{\bC}{\mathcal{C}}
\newcommand{\phit}{\phi_t}
\newcommand{\phiv}{\phi_x}
\newcommand{\se}{\text{SE}}
\newcommand{\HH}{\mathbb{H}}
\newcommand{\bYu}{\mathbf{Y}_{\text{uncertain}}}



==> tables/lp_only_fewshot.tex <==
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
% \begin{tabular}{rcccccccccccc}
% \begin{tabular}{rcccccccccccccccccc}
% \toprule 
%  & \multicolumn{6}{c}{RN50} & \multicolumn{6}{c}{RN101} & \\
% \cmidrule(lr){2-7} \cmidrule(lr){8-13} 
% \textbf{Dataset} & 1 & 2 & 4 & 8 & 16 & 32 & 1 & 2 & 4 & 8 & 16 & 32 \\
% \midrule
% \Pets     & 59.85 & 65.63 & 69.26 & 74.98 & 82.39 & 86.21 & 66.53 & 70.46 & 74.90 & 79.86 & 86.54 & 89.13 \\
% \Cars     & 36.94 & 46.56 & 56.31 & 65.28 & 72.32 & 77.07 & 42.82 & 54.76 & 63.51 & 71.71 & 78.56 & 82.28 \\
% \CUB      & 34.60 & 45.13 & 52.16 & 59.67 & 66.03 & 70.33 & 37.54 & 47.93 & 55.64 & 64.07 & 69.24 & 73.21 \\
% \DTD      & 33.83 & 43.51 & 47.82 & 55.64 & 61.86 & 71.38 & 36.97 & 45.16 & 50.53 & 58.51 & 64.04 & 71.54 \\
% \FGVC     & 15.75 & 18.81 & 24.00 & 30.36 & 36.84 & 42.81 & 17.73 & 22.44 & 27.15 & 32.61 & 39.33 & 44.88 \\
% \Food     & 53.03 & 60.30 & 66.24 & 72.45 & 75.63 & 77.87 & 57.22 & 65.48 & 70.93 & 77.29 & 80.42 & 82.30 \\
% \Flowers  & 67.17 & 80.14 & 88.52 & 93.14 & 93.76 & 93.82 & 72.04 & 82.37 & 89.72 & 93.92 & 94.47 & 94.45 \\
% \Imagenet & 33.67 & 40.59 & 47.42 & 52.98 & 56.72 & 57.36 & 36.33 & 44.29 & 51.50 & 57.36 & 61.07 & 62.33 \\
% \bottomrule
% % \cmidrule(lr){2-7} \cmidrule(lr){8-13}
% \end{tabular}%
\begin{tabular}{rcccccccccccccccccc}
\toprule 
\multicolumn{1}{l}{} & \multicolumn{6}{c}{RN50} & \multicolumn{6}{c}{RN101} & \multicolumn{6}{c}{ViT-B-32} \\
\cmidrule(lr){2-7} \cmidrule(lr){8-13} \cmidrule(lr){14-19} 
 & 1 & 2 & 4 & 8 & 16 & 32 & 1 & 2 & 4 & 8 & 16 & 32 & 1 & 2 & 4 & 8 & 16 & 32 \\ \midrule
\Pets & 59.85 & 65.63 & 69.26 & 74.98 & 82.39 & 86.21 & 66.53 & 70.46 & 74.90 & 79.86 & 86.54 & 89.13 & 69.58 & 75.69 & 80.46 & 83.16 & 86.81 & 88.80 \\
\Cars & 36.94 & 46.56 & 56.31 & 65.28 & 72.32 & 77.07 & 42.82 & 54.76 & 63.51 & 71.71 & 78.56 & 82.28 & 37.68 & 53.96 & 62.22 & 69.07 & 75.03 & 78.91 \\
\CUB & 34.60 & 45.13 & 52.16 & 59.67 & 66.03 & 70.33 & 37.54 & 47.93 & 55.64 & 64.07 & 69.24 & 73.21 & 40.54 & 51.55 & 56.61 & 64.17 & 69.33 & 72.70 \\
\DTD & 33.83 & 43.51 & 47.82 & 55.64 & 61.86 & 71.38 & 36.97 & 45.16 & 50.53 & 58.51 & 64.04 & 71.54 & 34.68 & 43.56 & 53.30 & 60.53 & 65.43 & 72.23 \\
\FGVC & 15.75 & 18.81 & 24.00 & 30.36 & 36.84 & 42.81 & 17.73 & 22.44 & 27.15 & 32.61 & 39.33 & 44.88 & 18.18 & 22.80 & 26.37 & 31.26 & 38.25 & 44.13 \\
\Food & 53.03 & 60.30 & 66.24 & 72.45 & 75.63 & 77.87 & 57.22 & 65.48 & 70.93 & 77.29 & 80.42 & 82.30 & 57.75 & 71.18 & 75.38 & 79.26 & 80.90 & 81.93 \\
\Flowers & 67.17 & 80.14 & 88.52 & 93.14 & 93.76 & 93.82 & 72.04 & 82.37 & 89.72 & 93.92 & 94.47 & \texttt{94.45} & 66.94 & 83.33 & 89.23 & 93.64 & 94.42 & \texttt{94.28} \\
\Imagenet & 33.67 & 40.59 & 47.42 & 52.98 & 56.72 & 57.36 & 36.33 & 44.29 & 51.50 & 57.36 & 61.07 & 62.33 & 44.64 & 52.41 & 56.35 & 59.60 & \texttt{53.77} & \texttt{57.49} \\
\midrule
\multicolumn{19}{c}{} \\
\midrule
% \end{tabular}%
% }
% \vspace{5cm}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{rcccccccccccccccccc}
% \toprule
 & \multicolumn{6}{c}{ViT-B-16} & \multicolumn{6}{c}{ViT-L-14} & \multicolumn{6}{c}{ \NNC{}}\\
\cmidrule(lr){2-7} \cmidrule(lr){8-13} \cmidrule(lr){14-19} 
 & 1 & 2 & 4 & 8 & 16 & 32 & 1 & 2 & 4 & 8 & 16 & 32 & 1 & 2 & 4 & 8 & 16 & 32 \\
 \midrule
\Pets & 79.39 & 81.96 & 85.04 & 88.33 & 91.41 & 92.56 & 82.34 & 85.85 & 87.71 & 90.76 & 93.57 & 94.66 & 94.09 & 94.03 & 93.81 & 94.16 & 94.19 & 94.19 \\
\Cars & 50.33 & 63.77 & 70.31 & 76.93 & 81.76 & 82.17 & 61.93 & 72.44 & 79.55 & 84.54 & 87.09 & 87.30 & - &  &  &  &  &  \\
\CUB & 47.46 & 60.79 & 66.60 & 71.26 & 76.56 & 80.43 & 52.83 & 65.34 & 73.44 & 79.43 & 82.78 & 84.76 & - &  &  &  &  &  \\
\DTD & 35.69 & 48.46 & 55.16 & 62.29 & 68.78 & 75.59 & 45.16 & 52.61 & 60.69 & 66.60 & 72.45 & 78.56 & - &  &  &  &  &  \\
\FGVC & 21.75 & 28.05 & 33.09 & 40.05 & 46.38 & 52.42 & 30.15 & 38.10 & 45.21 & 51.94 & 58.18 & 62.50 & - &  &  &  &  &  \\
\Food & 65.56 & 78.73 & 83.23 & 86.46 & 87.81 & 88.37 & 75.09 & 83.12 & 88.65 & 90.99 & 92.34 & 92.88 & - &  &  &  &  &  \\
\Flowers & 74.19 & 88.57 & 94.44 & 96.21 & 96.39 & 96.47 & 78.57 & 89.64 & 95.54 & 97.17 & 97.54 & 97.79 & - &  &  &  &  &  \\
\Imagenet & 51.22 & 59.09 & 63.07 & 65.68 & \texttt{61.08} & \texttt{63.14} & 60.72 & 67.51 & 71.34 & \texttt{65.49} & \texttt{66.37} & \texttt{70.69} & - &  &  &  &  & \\
\bottomrule
\end{tabular}%
% \begin{tabular}{rcccccccccccccccccc}
% \toprule
% % \cmidrule(lr){2-7} \cmidrule(lr){8-13} \cmidrule(lr){14-19}
%  & \multicolumn{6}{c}{ViT-B-32} & \multicolumn{6}{c}{ViT-B-16} & \multicolumn{6}{c}{ViT-L-14} \\
% \cmidrule(lr){2-7} \cmidrule(lr){8-13} \cmidrule(lr){14-19}
% \textbf{Dataset} & 1 & 2 & 4 & 8 & 16 & 32 & 1 & 2 & 4 & 8 & 16 & 32 & 1 & 2 & 4 & 8 & 16 & 32 \\ 
% \midrule
% \Pets & 69.58 & 75.69 & 80.46 & 83.16 & 86.81 & 88.80 & 79.39 & 81.96 & 85.04 & 88.33 & 91.41 & 92.56 & 82.34 & 85.85 & 87.71 & 90.76 & 93.57 & 94.66 \\
% \Cars & 37.68 & 53.96 & 62.22 & 69.07 & 75.00 & 72.79 & 50.33 & 63.77 & 70.31 & 76.93 & 81.76 & 82.17 & 61.93 & 72.44 & 79.55 & 84.54 & 82.28 & 84.94 \\
% \CUB & 40.54 & 51.55 & 56.61 & 64.17 & 69.33 & 72.70 & 47.46 & 60.79 & 66.60 & 71.26 & 76.56 & 80.43 & 52.83 & 65.34 & 73.44 & 79.43 & 82.78 & 84.76 \\
% \DTD & 34.68 & 43.56 & 53.30 & 60.53 & 65.43 & 72.23 & 35.69 & 48.46 & 55.16 & 62.29 & 68.78 & 75.59 & 45.16 & 52.61 & 60.69 & 66.60 & 72.45 & 78.56 \\
% \FGVC & 18.18 & 22.80 & 26.37 & 31.26 & 38.25 & 44.13 & 21.75 & 28.05 & 33.09 & 40.05 & 46.38 & 52.42 & 30.15 & 38.10 & 45.21 & 51.94 & 58.18 & 62.50 \\
% \Food & 57.75 & 71.18 & 75.38 & 79.26 & 80.90 & 81.93 & 65.56 & 78.73 & 83.23 & 86.46 & 87.81 & 88.37 & 75.09 & 83.12 & 88.65 & 90.99 & 92.34 & 92.88 \\
% \Flowers & 66.94 & 83.33 & 89.23 & 93.64 & 94.42 & 94.28 & 74.19 & 88.57 & 94.44 & 96.21 & 96.39 & 96.47 & 78.57 & 89.64 & 95.54 & 97.17 & 97.54 & 97.79 \\
% \Imagenet & 44.64 & 52.41 & 56.35 & 59.60 & 53.77 & 57.49 & 51.22 & 59.09 & 63.07 & 65.68 & 61.08 & 63.14 & 60.72 & 67.51 & 71.34 & 65.49 & 66.37 & 70.69 \\
% % \cmidrule(lr){2-7} \cmidrule(lr){8-13} \cmidrule(lr){14-19}
% \bottomrule
% \end{tabular}%
}
\caption{\CRO{CODING last results} FewShot linear probe}
\label{tab:fs}
\end{table*}

==> tables/variability_per_dataset.tex <==
\begin{table*}[]

\centering

\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{ccccccccc}
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
\multicolumn{1}{l}{} & \multicolumn{4}{c}{RN50} & \multicolumn{4}{c}{RN101} \\ 
\multicolumn{1}{l}{} & NoNorm & 1st order & L2-Norm & \begin{tabular}[c]{@{}c@{}}1st order\\ L2-Norm\end{tabular} & NoNorm & 1st order & L2-Norm & \begin{tabular}[c]{@{}c@{}}1st order\\ L2-Norm\end{tabular} \\ \cmidrule(lr){2-5} \cmidrule(lr){6-9}
Pets & - & 25.68 & 24.79 & 32.58 & - & 22.22 & 22.17 & 28.35 \\
Cars & - & 54.12 & 53.71 & 57.62 & - & 47.53 & 47.14 & 51.47 \\
Cub & - & 52.96 & 52.63 & 59.83 & - & 48.50 & 48.38 & 64.04 \\
Dtd & - & 33.77 & 32.11 & 41.01 & - & 33.11 & 30.90 & 47.11 \\
FGVC-Aircraft & - & 62.02 & 65.57 & 71.05 & - & 61.12 & 62.91 & 75.63 \\
Food & - & 35.08 & 33.41 & 38.74 & - & 31.95 & 29.45 & 39.74 \\
Flowers & - & 36.51 & 34.91 & 42.83 & - & 36.63 & 32.47 & 58.38 \\
ImageNet-1k & - & 38.73 & 38.49 & - & - & 36.57 & 35.37 & - \\ \cmidrule(lr){2-5} \cmidrule(lr){6-9}
\end{tabular}%
}

\resizebox{\textwidth}{!}{
\begin{tabular}{ccccccccccccc}
 \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
\multicolumn{1}{l}{} & \multicolumn{4}{c}{ViT-B-32} & \multicolumn{4}{c}{ViT-B-16} & \multicolumn{4}{c}{ViT-L-14} \\
\multicolumn{1}{l}{} & NoNorm & 1st order & L2-Norm & \begin{tabular}[c]{@{}c@{}}1st order\\ L2-Norm\end{tabular} & NoNorm & 1st order & L2-Norm & \begin{tabular}[c]{@{}c@{}}1st order\\ L2-Norm\end{tabular} & NoNorm & 1st order & L2-Norm & \begin{tabular}[c]{@{}c@{}}1st order\\ L2-Norm\end{tabular} \\  \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
Pets & - & 23.04 & 19.15 & 31.48 & - & 18.55 & 16.52 & 25.09 & - & 12.48 & 10.97 & 15.19 \\
Cars & - & 49.73 & 49.94 & 55.72 & - & 40.07 & 40.36 & 46.36 & - & 29.62 & 30.33 & 32.23 \\
Cub & - & 47.65 & 47.24 & 58.46 & - & 41.72 & 43.48 & 55.73 & - & 34.93 & 35.41 & 42.53 \\
Dtd & - & 32.46 & 31.13 & 45.87 & - & 29.69 & 28.49 & 40.50 & - & 25.40 & 24.51 & 32.55 \\
FGVC-Aircraft & - & 63.04 & 62.44 & 69.59 & - & 54.52 & 56.55 & 66.51 & - & 47.76 & 47.11 & 53.54 \\
Food & - & 29.39 & 26.70 & 32.95 & - & 21.84 & 20.61 & 24.42 & - & 13.81 & 13.39 & 15.78 \\
Flowers & - & 34.73 & 31.71 & 44.78 & - & 27.20 & 25.07 & 33.80 & - & 18.47 & 18.87 & 23.17 \\
ImageNet-1k & - & 34.99 & 34.06 & - & - & 28.91 & 27.96 & - & - & 21.46 & 21.27 & - \\  \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
\end{tabular}%
}

\caption{Variability of the predictions after applying augmentations}
\label{tab:variability_per_class}
\end{table*}

==> tables/zs_delta_accuracy_per_augmentations.tex <==
\begin{table*}[]

\centering

\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{ccccccccc}
 \cmidrule(lr){2-5} \cmidrule(lr){6-9}
\multicolumn{1}{l}{} & \multicolumn{4}{c}{RN50} & \multicolumn{4}{c}{RN101} \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{NoNorm} & \multicolumn{1}{l}{1st order} & \multicolumn{1}{l}{L2-Norm} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}1st order\\ L2-Norm\end{tabular}} & \multicolumn{1}{l}{NoNorm} & \multicolumn{1}{l}{1st order} & \multicolumn{1}{l}{L2-Norm} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}1st order\\ L2-Norm\end{tabular}} \\ 
 \cmidrule(lr){2-5} \cmidrule(lr){6-9}
resize crop & - & -11.88 & -11.92 & \textbf{-10.09} & - & -10.84 & -11.40 & \textbf{-4.47} \\
flip-resize & - & -3.35 & -2.61 & \textbf{-1.05} & - & -2.21 & -2.88 & \textbf{4.08} \\
flip-resize crop & - & -12.02 & -12.05 & \textbf{-10.16} & - & -11.05 & -11.58 & \textbf{-4.69} \\
grayscale-resize & - & -26.07 & -24.01 & \textbf{-21.96} & - & -22.81 & -22.13 & \textbf{-14.92} \\
grayscale-resize crop & - & -34.80 & -33.79 & \textbf{-32.02} & - & -31.49 & -32.68 & \textbf{-25.58} \\
color jitter-resize & - & -13.98 & -13.46 & \textbf{-11.98} & - & -11.72 & -12.56 & \textbf{-5.65} \\
color jitter-resize crop & - & -23.59 & -23.58 & \textbf{-21.98} & - & -21.04 & -22.58 & \textbf{-15.64} \\
gaussian blur-resize & - & -6.33 & -5.63 & \textbf{-4.23} & - & -5.02 & -5.34 & \textbf{1.51} \\
gaussian blur-resize crop & - & -17.02 & -16.61 & \textbf{-15.14} & - & -15.89 & -16.14 & \textbf{-9.47} \\ 
 \cmidrule(lr){2-5} \cmidrule(lr){6-9}
\end{tabular}%
}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccccccccc}
 \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
\multicolumn{1}{l}{} & \multicolumn{4}{c}{ViT-B-32} & \multicolumn{4}{c}{ViT-B-16} & \multicolumn{4}{c}{ViT-L-14} \\
\multicolumn{1}{l}{} & \multicolumn{1}{l}{NoNorm} & \multicolumn{1}{l}{1st order} & \multicolumn{1}{l}{L2-Norm} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}1st order\\ L2-Norm\end{tabular}} & \multicolumn{1}{l}{NoNorm} & \multicolumn{1}{l}{1st order} & \multicolumn{1}{l}{L2-Norm} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}1st order\\ L2-Norm\end{tabular}} & \multicolumn{1}{l}{NoNorm} & \multicolumn{1}{l}{1st order} & \multicolumn{1}{l}{L2-Norm} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}1st order\\ L2-Norm\end{tabular}} \\
 \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
resize crop & - & -9.91 & -9.60 & \textbf{-6.46} & - & -9.36 & -9.24 & \textbf{-7.66} & - & -8.16 & -7.85 & \textbf{-7.27} \\
flip-resize & - & -3.00 & -2.90 & \textbf{0.03} & - & -1.38 & -1.84 & \textbf{-0.44} & - & -1.69 & -1.70 & \textbf{-1.18} \\
flip-resize crop & - & -10.09 & -9.62 & \textbf{-6.57} & - & -9.53 & -9.37 & \textbf{-7.82} & - & -8.30 & -8.13 & \textbf{-7.49} \\
grayscale-resize & - & -27.78 & -25.49 & \textbf{-22.43} & - & -22.54 & -19.67 & \textbf{-18.30} & - & -16.08 & -14.67 & \textbf{-13.70} \\
grayscale-resize crop & - & -35.44 & -33.79 & \textbf{-30.78} & - & -32.29 & -30.05 & \textbf{-28.55} & - & -26.43 & -24.82 & \textbf{-24.13} \\
color jitter-resize & - & -13.42 & -12.72 & \textbf{-9.51} & - & -9.58 & -9.02 & \textbf{-7.48} & - & -6.54 & -6.58 & \textbf{-6.09} \\
color jitter-resize crop & - & -21.39 & -20.81 & \textbf{-17.57} & - & -19.15 & -18.56 & \textbf{-16.91} & - & -15.00 & -14.74 & \textbf{-14.31} \\
gaussian blur-resize & - & -4.95 & -4.85 & \textbf{-1.96} & - & -3.14 & -3.33 & \textbf{-2.26} & - & -2.67 & -2.84 & \textbf{-2.52} \\
gaussian blur-resize crop & - & -13.31 & -12.81 & \textbf{-9.79} & - & -12.70 & -12.28 & \textbf{-10.97} & - & -10.62 & -10.08 & \textbf{-9.65} \\ 
 \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
\end{tabular}%
}
\caption{delta accuracy of the predictions per augmentations}
\label{tab:delta_accu_per_aug}
\end{table*}

==> tables/zs_delta_accuracy_per_dataset.tex <==
\begin{table*}[]

\centering

\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{ccccccccc}
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
\multicolumn{1}{l}{} & \multicolumn{4}{c}{RN50} & \multicolumn{4}{c}{RN101} \\
\multicolumn{1}{l}{} & NoNorm & 1st order & L2-Norm & \begin{tabular}[c]{@{}c@{}}1st order\\ L2-Norm\end{tabular} & NoNorm & 1st order & L2-Norm & \begin{tabular}[c]{@{}c@{}}1st order\\ L2-Norm\end{tabular} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
Pets & - & \textbf{-12.91} & -13.50 & -14.09 & - & \textbf{-11.77} & -13.29 & -12.54 \\
Cars & - & -17.07 & \textbf{-15.52} & -17.13 & - & -15.54 & -15.58 & \textbf{-14.65} \\
Cub & - & -12.72 & -12.71 & \textbf{-9.52} & - & -10.85 & -12.90 & \textbf{-2.09} \\
Dtd & - & -3.72 & -3.15 & \textbf{-2.19} & - & -4.30 & -3.85 & \textbf{-2.25} \\
FGVC-Aircraft & - & -2.05 & -2.45 & \textbf{-1.49} & - & -1.87 & -2.44 & \textbf{0.35} \\
Food & - & -17.69 & -17.37 & \textbf{-14.50} & - & -16.06 & -16.43 & \textbf{-8.78} \\
Flowers & - & -12.47 & -12.43 & \textbf{-11.83} & - & -8.77 & -10.30 & \textbf{4.86} \\
ImageNet-1k & - & -10.86 & -11.08 & - & - & -10.28 & -10.32 & - \\ 
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
\end{tabular}%
}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccccccccc}
 \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
\multicolumn{1}{l}{} & \multicolumn{4}{c}{ViT-B-32} & \multicolumn{4}{c}{ViT-B-16} & \multicolumn{4}{c}{ViT-L-14} \\
\multicolumn{1}{l}{} & NoNorm & 1st order & L2-Norm & \begin{tabular}[c]{@{}c@{}}1st order\\ L2-Norm\end{tabular} & NoNorm & 1st order & L2-Norm & \begin{tabular}[c]{@{}c@{}}1st order\\ L2-Norm\end{tabular} & NoNorm & 1st order & L2-Norm & \begin{tabular}[c]{@{}c@{}}1st order\\ L2-Norm\end{tabular} \\
 \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
Pets & - & -11.30 & -10.64 & \textbf{-10.45} & - & -9.98 & -8.70 & \textbf{-7.70} & - & -7.65 & \textbf{-7.01} & -7.64 \\
Cars & - & \textbf{-15.35} & -15.82 & -15.37 & - & -12.16 & -12.48 & \textbf{-11.75} & - & -11.93 & -12.57 & \textbf{-11.69} \\
Cub & - & -12.61 & -12.93 & \textbf{-7.05} & - & -11.52 & -12.19 & \textbf{-6.11} & - & -12.04 & -11.46 & \textbf{-9.56} \\
Dtd & - & -3.73 & \textbf{-3.09} & -5.83 & - & \textbf{-1.54} & -1.66 & -4.42 & - & -3.09 & \textbf{-2.42} & -3.12 \\
FGVC-Aircraft & - & -1.98 & -1.68 & \textbf{-1.35} & - & -2.21 & -2.38 & \textbf{-1.30} & - & -3.80 & \textbf{-3.41} & -3.55 \\
Food & - & -14.91 & -14.10 & \textbf{-9.16} & - & -12.89 & -12.46 & \textbf{-10.97} & - & -8.52 & -8.29 & \textbf{-7.74} \\
Flowers & - & -10.48 & -9.60 & \textbf{-8.22} & - & -9.15 & \textbf{-7.64} & -8.19 & - & -7.41 & \textbf{-7.11} & -7.61 \\
ImageNet-1k & - & -9.66 & -9.37 & - & - & -8.53 & -8.23 & - & - & -7.31 & -7.10 & - \\
 \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13}
\end{tabular}%
}
\caption{delta accuracy of the predictions after applying augmentations}
\label{tab:delta_accu}
\end{table*}

==> tables/zs_table.tex <==
\begin{table}[t]
\centering
\resizebox{0.49\textwidth}{!}{
\begin{tabular}{ccccccc}
\toprule
 & RN50 & RN101 & ViT-B-32 & ViT-B-16 & ViT-L-14 & upperbound \\
\midrule
Pets & 85.80 & 86.86 & 87.46 & 89.07 & 93.59 & 98.06 \\
Cars & 54.22 & 61.12 & 59.73 & 64.61 & 77.75 & 90.85 \\
Cub & 46.57 & 49.64 & 52.99 & 55.28 & 62.06 & 81.20 \\
Dtd & 41.22 & 43.67 & 43.99 & 45.11 & 55.32 & 69.63 \\
FGVC-Aircraft & 17.07 & 18.63 & 19.65 & 24.39 & 31.71 & 52.09 \\
Food & 77.91 & 81.86 & 82.58 & 87.91 & 92.32 & 96.60 \\
Flowers & 66.12 & 65.20 & 66.48 & 71.43 & 79.05 & 86.32 \\
ImageNet-1k & 59.84 & 62.28 & 63.35 & 68.34 & 75.54 & 85.30 \\
\bottomrule
\end{tabular}
}
\caption{Zero-shot accuracy performance for multiple datasets using different backbones and its upperbound if we perfectly combine them.}
\label{tab:zs-table}
\end{table}
